Explicit Visual Prompting for Universal Foreground Segmentations

Foreground segmentation is a fundamental problem in computer vision, which includes salient object detection, forgery detection, defocus blur detection, shadow detection, and camouflage object detection. Previous works have typically relied on domain-specific solutions to address accuracy and robustness issues in those applications. In this paper, we present a unified framework for a number of foreground segmentation tasks without any task-specific designs. We take inspiration from the widely-used pre-training and then prompt tuning protocols in NLP and propose a new visual prompting model, named Explicit Visual Prompting (EVP). Different from the previous visual prompting which is typically a dataset-level implicit embedding, our key insight is to enforce the tunable parameters focusing on the explicit visual content from each individual image, i.e., the features from frozen patch embeddings and high-frequency components. Our method freezes a pre-trained model and then learns task-specific knowledge using a few extra parameters. Despite introducing only a small number of tunable parameters, EVP achieves superior performance than full fine-tuning and other parameter-efficient fine-tuning methods. Experiments in fourteen datasets across five tasks show the proposed method outperforms other task-specific methods while being considerably simple. The proposed method demonstrates the scalability in different architectures, pre-trained weights, and tasks. The code is available at: https://github.com/NiFangBaAGe/Explicit-Visual-Prompt.

==> figs/archs.tex <==

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/images/overview.pdf}
    \vspace{-1em}
    \caption{Overview of the proposed model.}
    \label{fig:overview}
\end{figure*}


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/images/adaptor.pdf}
    \vspace{-1em}
    \caption{
    The procedure to generate high-frequency components~(top).
    The architecture of the proposed explicit visual prompting with adaptor~(bottom). We use the \textit{Embedding Tune} and the \textit{HFC Tune} to tune the extracted features. The Adaptor is designed to merge these features. }
    \label{fig:adaptor}
\end{figure}


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/images/adaptor_new.pdf}
    \vspace{-1em}
    \caption{
    The proposed Fourier MLP~(top).
    The architecture of the proposed explicit visual prompting with Frequency Enhanced Adaptor~(bottom). }
    \label{fig:adaptor_new}
\end{figure}

==> figs/cod.tex <==
% % Figure SOTA
\begin{figure*}[t]
  \captionsetup[subfigure]{position=b}
  \centering

  \setlength{\tabcolsep}{0pt}% Remove column gap in tabular
  \subcaptionbox{Input}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/input/camourflage_00183.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/input/camourflage_00269.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/input/camourflage_00478.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{GT}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/gt/camourflage_00183.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/gt/camourflage_00269.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/gt/camourflage_00478.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{Ours}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/ours/camourflage_00183.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/ours/camourflage_00269.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/ours/camourflage_00478.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{SINet}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/sinet/camourflage_00183.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/sinet/camourflage_00269.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/sinet/camourflage_00478.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{PFNet}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/pfnet/camourflage_00183.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/pfnet/camourflage_00269.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/pfnet/camourflage_00478.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{JCOD}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/jcod/camourflage_00183.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/jcod/camourflage_00269.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/jcod/camourflage_00478.png}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{RankNet}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/ranknet/camourflage_00183.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/ranknet/camourflage_00269.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/cod/ranknet/camourflage_00478.png}
    \end{tabular}}
  \subcaptionbox{\scriptsize{Input}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/input/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/input/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/input/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{GT}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/gt/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/gt/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/gt/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{Ours}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/ours/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/ours/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/ours/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{ManTra}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/mantranet/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/mantranet/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/mantranet/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{SPAN}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/span/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/span/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/forgery/span/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%

\caption{(a)-(g)~Comparison with other state-of-the-art methods on CAMO~\cite{le2019anabranch} dataset for camouflaged object detection. We compare to SINet~\cite{fan2020camouflaged}, PFNEt~\cite{mei2021camouflaged}, JCOD~\cite{li2021uncertainty} and RankNet~\cite{lv2021simultaneously}. (h)-(l) Forgery detection results on CAISA~\cite{dong2013casia} dataset, we compare our method with ManTraNet~\cite{wu2019mantra} and SPAN~\cite{hu2020span}.}
\label{fig:cod_sota}
\end{figure*}



==> figs/defocus.tex <==
% % Figure SOTA
\begin{figure}[t]
  \captionsetup[subfigure]{position=b}
  \centering

  \setlength{\tabcolsep}{0pt}% Remove column gap in tabular
  \subcaptionbox{\scriptsize{Input}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/input/26.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/input/27.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/input/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{GT}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/gt/26.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/gt/27.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/gt/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{Ours}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/ours/26.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/ours/27.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/ours/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{BTBNet}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/btbnet/26.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/btbnet/27.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/btbnet/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{CENet}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/cenet/26.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/cenet/27.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/cenet/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{EFENet}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/efenet/26.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/efenet/27.jpg} \\[0.1em]
      \includegraphics[width=0.155\columnwidth, height=0.155\columnwidth]{images/defocus/efenet/93.jpg}
    \end{tabular}}%
    \vspace{-1em}
\caption{Comparison with state-of-the-art methods on CUHK~\cite{shi2014discriminative} dataset for defocus blur detection. We compare to BTBNet~\cite{zhao2019btbnet}, CENet~\cite{zhao2019cenet} and EFENet~\cite{zhao2021defocus}.}
\label{fig:defocus_sota}
\end{figure}


==> figs/exp.tex <==

\newcommand\wwthree{0.3\textwidth}
\newcommand\hhthree{0.3\textwidth}

\begin{figure*}[t]
\centering
\includegraphics[width=0.3\linewidth]{figs/exp/CAISA_F1.png}
\includegraphics[width=0.3\linewidth]{figs/exp/ISTD_BER.png}
\includegraphics[width=0.3\linewidth]{figs/exp/DUT_FMeasure.png}
\caption{Mask Ratio.}
\label{fig:mask_ratio}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.3\linewidth]{figs/exp/CAISA_Filter.png}
\includegraphics[width=0.3\linewidth]{figs/exp/ISTD_Filter.png}
\includegraphics[width=0.3\linewidth]{figs/exp/DUT_Filter.png}
\caption{Filter.}
\label{fig:filter}
\end{figure*}



==> figs/forgery.tex <==
% % Figure SOTA
\begin{figure}[t]
  \captionsetup[subfigure]{position=b}
  \centering

  \setlength{\tabcolsep}{0pt}% Remove column gap in tabular
  \subcaptionbox{\scriptsize{Input}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/input/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/input/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/input/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{GT}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/gt/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/gt/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/gt/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{Ours}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/ours/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/ours/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/ours/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{ManTraNet}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/mantranet/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/mantranet/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/mantranet/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{SPAN}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/span/Sp_D_CRN_A_ani0043_ani0041_0373.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/span/Sp_D_NND_A_nat0022_ani0063_0188.jpg} \\[0.1em]
      \includegraphics[width=0.185\columnwidth, height=0.185\columnwidth]{images/forgery/span/Sp_D_NND_A_nat0031_nat0096_0610.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \vspace{-1em}
\caption{Comparison with state-of-the-art methods on CAISA~\cite{dong2013casia} dataset for forgery detection. We compare to ManTraNet~\cite{wu2019mantra} and SPAN~\cite{hu2020span}.}
\label{fig:caisa_sota}
\end{figure}


% \newcommand\wwab{0.18\columnwidth}
% \newcommand\hhab{0.18\columnwidth}
% \captionsetup[figure]{font=small}
% \begin{figure}[t]
% \centering
% % input
% \subcaptionbox{}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/input/Sp_D_CRN_A_ani0043_ani0041_0373.jpg}}
% \subcaptionbox{}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/gt/Sp_D_CRN_A_ani0043_ani0041_0373.jpg}}
% \subcaptionbox{}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/ours/Sp_D_CRN_A_ani0043_ani0041_0373.jpg}}
% \subcaptionbox{}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/mantranet/Sp_D_CRN_A_ani0043_ani0041_0373.jpg}}
% \subcaptionbox{}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/span/Sp_D_CRN_A_ani0043_ani0041_0373.jpg}}

% \par\bigskip\vspace*{-2em}
% \subcaptionbox{
%         \label{img-0}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/input/Sp_D_NND_A_nat0022_ani0063_0188.jpg}}
% \subcaptionbox{
%         \label{img-1}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/gt/Sp_D_NND_A_nat0022_ani0063_0188.jpg}}
% \subcaptionbox{
%         \label{img-2}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/ours/Sp_D_NND_A_nat0022_ani0063_0188.jpg}}
% \subcaptionbox{
%         \label{img-3}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/mantranet/Sp_D_NND_A_nat0022_ani0063_0188.jpg}}
% \subcaptionbox{
%         \label{img-4}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/span/Sp_D_NND_A_nat0022_ani0063_0188.jpg}}

% \par\bigskip\vspace*{-2em}
% % \setcounter{subfigure}{0}% Reset subcaptionbox counter
% % \addtocounter{subfigure}{-10}
% \subcaptionbox{\scriptsize{Input}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/input/Sp_D_NND_A_nat0031_nat0096_0610.jpg}}
% \subcaptionbox{\scriptsize{Target}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/gt/Sp_D_NND_A_nat0031_nat0096_0610.jpg}}
% \subcaptionbox{\scriptsize{Ours}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/ours/Sp_D_NND_A_nat0031_nat0096_0610.jpg}}
% \subcaptionbox{\scriptsize{ManTraNet}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/mantranet/Sp_D_NND_A_nat0031_nat0096_0610.jpg}}
% \subcaptionbox{\scriptsize{SPAN}}{\centering\includegraphics[width=0.185\columnwidth, height=0.185\columnwidth,height=0.185\columnwidth]{images/forgery/span/Sp_D_NND_A_nat0031_nat0096_0610.jpg}}

% \caption{Comparison with state-of-the-art methods on CAISA dataset for forgery detection.}
% \label{fig:sota}
% \end{figure}
% \captionsetup[figure]{font=small}

==> figs/shadow.tex <==
% % Figure SOTA
\begin{figure*}[t]
  \captionsetup[subfigure]{position=b}
  \centering
  \setlength{\tabcolsep}{0pt}% Remove column gap in tabular
  \subcaptionbox{\scriptsize{Input}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/input/94-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/input/113-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/input/114-10.png}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{GT}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/gt/94-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/gt/113-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/gt/114-10.png}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{Ours}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/ours/94-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/ours/113-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/ours/114-10.png}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{DSD}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/dsd/94-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/dsd/113-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/dsd/114-10.png}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{MTMT}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/mtmt/94-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/mtmt/113-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/mtmt/114-10.png}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{FDRNet}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/fdrnet/94-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/fdrnet/113-2.png} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/shadow/fdrnet/114-10.png}
    \end{tabular}}%
\hspace{0.5em}%
  \subcaptionbox{\scriptsize{Input}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/input/26.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/input/27.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/input/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{GT}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/gt/26.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/gt/27.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/gt/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{Ours}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/ours/26.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/ours/27.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/ours/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{BTBNet}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/btbnet/26.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/btbnet/27.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/btbnet/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{CENet}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/cenet/26.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/cenet/27.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/cenet/93.jpg}
    \end{tabular}}%
  \hspace{0.0em}%
  \subcaptionbox{\scriptsize{EFENet}}{%
    \begin{tabular}{c}
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/efenet/26.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/efenet/27.jpg} \\[0.1em]
      \includegraphics[width=0.162\columnwidth, height=0.14\columnwidth]{images/defocus/efenet/93.jpg}
    \end{tabular}}%
    \hspace{0.0em}%
\caption{(a)-(f) Comparison with other methods~(DSD~\cite{zhao2021self}, MTMT~\cite{mtmt}, FDRNet~\cite{zhu2021mitigating}) on ISTD~\cite{wang2018stacked} dataset for shadow detection. (g)-(l)~Comparison with other methods on CUHK~\cite{shi2014discriminative} dataset for defocus blur detection, including BTBNet~\cite{zhao2019btbnet}, CENet~\cite{zhao2019cenet} and EFENet~\cite{zhao2021defocus}.}
\label{fig:shadow_sota}
\end{figure*}



==> figs/teaser.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/images/teaser_new.pdf}
    \caption{We propose a unified method for four low-level structure segmentation tasks: camouflaged object, forgery, shadow and defocus blur detection~(Top). Our approach relies on a pre-trained frozen transformer backbone that leverages explicit extracted features, \emph{e.g.}, the frozen embedded features and high-frequency components, to prompt knowledge. } %We also design the \textit{explicit visual prompting}, which utilizes explicit extracted features~(\eg, high-frequency components and the frozen embedded features) as prompting to tune.} %With only 5.7\% extra trainable parameters, our method achieves the state-of-the-art performance.}
    \label{fig:teaser}
\end{figure}
